On Computational Limits of Modern Hopfield Models: A Fine-Grained Complexity Analysis

We investigate the computational limits of the memory retrieval dynamics of modern Hopfield models from the fine-grained complexity analysis. Our key contribution is the characterization of a phase transition behavior in the efficiency of all possible modern Hopfield models based on the norm of patterns. Specifically, we establish an upper bound criterion for the norm of input query patterns and memory patterns. Only below this criterion, sub-quadratic (efficient) variants of the modern Hopfield model exist, assuming the Strong Exponential Time Hypothesis (SETH). To showcase our theory, we provide a formal example of efficient constructions of modern Hopfield models using low-rank approximation when the efficient criterion holds. This includes a derivation of a lower bound on the computational time, scaling linearly with $\max\{$# of stored memory patterns, length of input query sequence$\}$. In addition, we prove its memory retrieval error bound and exponential memory capacity.

==> 3exp.tex <==
To be filled.


\subsection{Data}



\subsubsection{Synthetic Dataset:}


\subsubsection{Realistic Dataset I:}


\subsubsection{Realistic Dataset II:}





\subsection{Benchmarks and Evaluation}


\subsection{Results}




==> notation.tex <==
\paragraph{Notations.} 
We denote (column) vectors by lower case bold letters, and matrices by upper case bold letters.
We write $\Braket{\ba,\bb}\coloneqq \ba^\sT \bb$ as the inner product for vectors $\ba,\bb$.
Let $\ba[i]$ denotes the $i$-th component of vector $\ba$.
The index set $\{1,\cdots,I\}$ is denoted by $[I]$, where $I\in\mathbb{N}_+$.
Let $\norm{\bA}_{\text{max}}\coloneqq\max_{i,j} \abs{\bA_{ij}}$ for any matrix $\bA$. 
We denote the memory patterns by $\bxi\in\R^d$ and the query pattern by $\bx\in\R^d$, and $\bm{\Xi}\coloneqq\[\bxi_1,\cdots,\bxi_M\]\in \R^{d\times M}$ as shorthand for stored memory patterns $\{\bxi_\mu\}_{\mu\in[M]}$.
We denote $\{\underline{\bm\tau}_{1}, \cdots, \underline{\bm\tau}_{d}\} \subset \R^{1\times n}$ for each row in the matrix $\bZ \in \R^{d\times n}$.

